High-order Joint Constituency and Dependency Parsing

This work revisits the topic of jointly parsing constituency and dependency trees, i.e., to produce compatible constituency and dependency trees simultaneously for input sentences, which is attractive considering that the two types of trees are complementary in representing syntax. The original work of Zhou and Zhao (2019) performs joint parsing only at the inference phase. They train two separate parsers under the multi-task learning framework (i.e., one shared encoder and two independent decoders). They design an ad-hoc dynamic programming-based decoding algorithm of $O(n^5)$ time complexity for finding optimal compatible tree pairs. Compared to their work, we make progress in three aspects: (1) adopting a much more efficient decoding algorithm of $O(n^4)$ time complexity, (2) exploring joint modeling at the training phase, instead of only at the inference phase, (3) proposing high-order scoring components to promote constituent-dependency interaction. We conduct experiments and analysis on seven languages, covering both rich-resource and low-resource scenarios. Results and analysis show that joint modeling leads to a modest overall performance boost over separate modeling, but substantially improves the complete matching ratio of whole trees, thanks to the explicit modeling of tree compatibility.

==> figure_ana.tex <==

\begin{figure}[htb!]
  \centering
  \small
  \pgfkeys{/pgf/inner sep=0.1em}
    \subfigure[Correct dependency parsing from \textsc{Joint1o}]{
        \label{fig:ana-dep-c}
        \includegraphics[scale=0.18]{figures/dep_r_w_con.png}
            
    }
    \\
    \subfigure[Wrong dependency parsing from \textsc{Mtl}]{
        \label{fig:ana-dep-w}
        \includegraphics[scale=0.18]{figures/dep_w_w_con.png}
            
    }
  \caption{Partial parsing results from different models. The correct constituents are parsed by both \textsc{Joint1o} and \textsc{Mtl}, i.e., $(\textit{WHADJP}, how\ many)$ and $(\textit{WHANP}, how\ many\ more)$. 
  }
  \label{fig:ana}
\end{figure}


==> figure_tree.tex <==
figure_
\begin{figure*}[htb!]
  \centering
  \small
  \pgfkeys{/pgf/inner sep=0.1em}
    \subfigure[Lexicalized tree (head-binarized)]{
        \label{fig:lex}    
        \begin{tikzpicture}[
              level distance=22.5pt,
              every tree node/.style={align=center,anchor=base},
              frontier/.style={distance from root=125pt},
              case_blue/.style={midnightblue, fill=midnightblue!20, draw=midnightblue, thick, fill opacity=1., text opacity=1., rounded corners=1mm,align=center, minimum size=4mm},
              edge from parent/.style={thick, draw, black!70, edge from parent path={(\tikzparentnode.south) {[rounded corners=0.5pt]-- ($(\tikzchildnode |- \tikzparentnode.south) + (0, -5pt)$) -- (\tikzchildnode)}}}
              ]
        \Tree
            [.\node[case_blue]{S[take]}; 
                \edge[midnightblue, -{Stealth[width=1.5mm,length=1.3mm]}];
                [.\node[case_blue]{NP[laws]}; 
                    [.DT[The] The$_0$ ] 
                    [.NNS[laws] laws$_1$ ]
                ]
                [.VP[take] 
                    [.VP$^\ast$[take] 
                        [.VBP[take] take$_2$ ]
                        [.NN[effect] effect$_3$ ]
                    ]
                    [.NP[month] 
                        [.JJ[next] next$_4$ ]
                        [.NN[month] month$_5$ ]
                    ]
                    ]
                ]
            ];
        \end{tikzpicture}
    }
    \hfill
    \begin{minipage}[b]{0.37\textwidth}
    \subfigure[Constituency tree]{
        \label{fig:cosnt}    
        \begin{tikzpicture}[
              level distance=22.5pt,
              every tree node/.style={align=center,anchor=base},
              frontier/.style={distance from root=62pt},
              case_red/.style={brickred, fill=brickred!20, draw=brickred, thick, fill opacity=1., text opacity=1., rounded corners=1mm,align=center, minimum size=4mm},
              case_blue/.style={midnightblue, fill=midnightblue!20, draw=midnightblue, thick, fill opacity=1., text opacity=1., rounded corners=1mm,align=center, minimum size=4mm},
              edge from parent/.style={thick, draw, black!70, edge from parent path={(\tikzparentnode.south) {[rounded corners=0.5pt]-- ($(\tikzchildnode |- \tikzparentnode.south) + (0, -5pt)$) -- (\tikzchildnode)}}} 
              ]
        \Tree
            [.S 
                [.NP 
                    The 
                    laws
                ]
                [.VP 
                    take
                    effect
                    [.NP
                        next
                        month
                    ]
                ]
            ];
        \end{tikzpicture}
    }
    \\
        \subfigure[Dependency tree]{
        \label{fig:dep}
        \begin{dependency}[hide label]
            \begin{deptext} [row sep=0.2cm, column sep=0.01cm]
            \$ \& The \& \textcolor{midnightblue}{laws} \& \textcolor{midnightblue}{take} \& effect \& next \& month \\
            \end{deptext}
                        
            \depedge[edge start x offset=0pt, edge style={black!70, thick}, edge height=4ex]{4}{1}{}
            \depedge[arc angle=50, edge style={black!70, thick}, edge height=3ex]{2}{3}{Head}
            \depedge[arc angle=50, edge below, style={midnightblue, thick}, edge height=2ex]{3}{4}{}
            \depedge[arc angle=50, edge end x offset=2pt, edge style={black!70, thick}, edge height=3ex]{5}{4}{}
            \depedge[edge style={black!70, thick}, edge height=3ex]{6}{7}{}
            \depedge[edge start x offset=6pt, edge end x offset=-2pt, edge style={black!70, thick}, edge height=4ex]{7}{4}{}

            \wordgroup[color=midnightblue,thick,fill=midnightblue!20]{1}{3}{4}{}
            

        \end{dependency}
    }
    \end{minipage}

  \caption{An example sentence with three kinds of syntactic trees. All lexicalized constituents are annotated by head words with $\left[ \cdot \right]$ and the fictional constituent labels resulting from binarization all end with "$*$" symbol. All dependency labels are omitted for simplicity. With the head-binarization, we can observe that the lexicalized tree is structurally compatible with the dependency tree. }
  \label{fig:lex-example}
\end{figure*}

